Plasmoid-dominated Turbulent Reconnection in a Low $\beta$ Plasma

Properties of plasmoid-dominated turbulent reconnection in a low-$\beta$ background plasma are investigated by resistive magnetohydrodynamic (MHD) simulations. In the $\beta_{\rm in} < 1$ regime, where $\beta_{\rm in}$ is plasma $\beta$ in the inflow region, the reconnection site is dominated by shocks and shock-related structures and plasma compression is significant. The effective reconnection rate increases from $0.01$ to $0.02$ as $\beta_{\rm in}$ decreases. We hypothesize that plasma compression allows faster reconnection rate, and then we estimate a speed-up factor, based on a compressible MHD theory. We validate our prediction by a series of MHD simulations. These results suggest that the plasmoid-dominated reconnection can be twice faster than expected in the $\beta \ll 1$ environment in a solar corona.

==> ancillary_files/Makefile <==
### NAOJ/XC
F90 = ftn -hnoomp # OpenMP OFF
# F90 = ftn -homp   # OpenMP ON
### JAXA/FX100
# F90 = f90sjx -Umpi -Uflat

OBJS = model.o set_dt.o set_dt2.o set_eta.o u2v.o input.o output.o \
	rk21.o rk22.o step1.o step2.o bc.o bc_vlvr_g.o \
	flux_solver.o limiter.o flux_resistive.o flux_glm.o glm_ss.o
OBJP2= modelp2.o mpibc2.o mpibc_vlvr_f2.o bc_vlvr_g2.o  mpiinput.o mpioutput.o outflow.o

all: run runp2

# serial version
run : main.o $(OBJS)
	$(F90) -o a.out main.o $(OBJS)

# parallel version
runp2 : mainp2.o $(OBJS) $(OBJP2)
	$(F90) -o ap2.out mainp2.o $(OBJS) $(OBJP2)

# parallel version: artificial impact added
runp2noise : mainp2noise.o $(OBJS) $(OBJP2) modelp2noise.o
	$(F90) -o ap2noise.out mainp2noise.o $(OBJS) $(OBJP2) modelp2noise.o

%.o: %.f90 param.h
	$(F90) $(FFLAGS) -c $<

clean :
	rm -f *.out *.o data/*.dat data/*.dat.restart

